The Direct-Connectedness Function in the Random Connection Model

We investigate expansions for connectedness functions in the random connection model of continuum percolation in powers of the intensity. Precisely, we study the pair-connectedness and the direct-connectedness functions, related to each other via the Ornstein-Zernike equation. We exhibit the fact that the coefficients of the expansions consist of sums over connected and $2$-connected graphs. In the physics literature, this is known to be the case more generally for percolation models based on Gibbs point processes and stands in analogy to the formalism developed for correlation functions in liquid-state statistical mechanics. We find a representation of the direct-connectedness function and bounds on the intensity which allow us to pass to the thermodynamic limit. In some cases (e.g., in high dimensions), the results are valid in almost the entire subcritical regime. Moreover, we relate these expansions to the physics literature and we show how they coincide with the expression provided by the lace expansion.

==> OZEbib2.tex <==
@incollection {brydges1986leshouches,
    AUTHOR = {Brydges, D. C.},
     TITLE = {A short course on cluster expansions},
 BOOKTITLE = {Ph\'{e}nom\`enes critiques, syst\`emes al\'{e}atoires, th\'{e}ories de jauge,
              {P}art {I}, {II} ({L}es {H}ouches, 1984)},
     PAGES = {129--183},
 PUBLISHER = {North-Holland, Amsterdam},
      YEAR = {1986}
}

@Article{BrySpe85,
 Author = {D. C. {Brydges} and T. {Spencer}},
 Title = {{Self-avoiding walk in 5 or more dimensions}},
 FJournal = {{Communications in Mathematical Physics}},
 Journal = {{Commun. Math. Phys.}},
 ISSN = {0010-3616; 1432-0916/e},
 Volume = {97},
 Number = {1-2},
 Pages = {125--148},
 Year = {1985},
 Publisher = {Springer, Berlin/Heidelberg},
 MSC2010 = {60K35 81P20 60G50},
 Zbl = {0575.60099}
}

@ARTICLE{ConDeAngFor77,
       author = {{Coniglio}, A. and {DeAngelis}, U. and {Forlani}, A.},
        title = "{Pair connectedness and cluster size}",
      journal = {J. Phys. A},
      fjournal = {Journal of Physics A Mathematical General},
         year = "1977",
        month = "Jul",
       volume = {10},
       number = {7},
        pages = {1123-1139},
          doi = {10.1088/0305-4470/10/7/011},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1977JPhA...10.1123C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article {campanino-ioffe2002,
    AUTHOR = {Campanino, M. and Ioffe, D.},
     TITLE = {Ornstein-{Z}ernike theory for the {B}ernoulli bond percolation
              on {$\Bbb Z^d$}},
   JOURNAL = {Ann. Probab.},
  FJOURNAL = {The Annals of Probability},
    VOLUME = {30},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {652--682}
}


@ARTICLE{Hil55,
       author = {{Hill}, T. L.},
        title = "{Molecular Clusters in Imperfect Gases}",
      journal = {J. Chem. Phys.},
      fjournal = {The Journal Of Chemical Physics},
         year = "1955",
        month = "Apr",
       volume = {23},
       number = {4},
        pages = {617-622},
          doi = {10.1063/1.1742067},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1955JChPh..23..617H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{HarSla90,
 Author = {T. {Hara} and G. {Slade}},
 Title = {{Mean-field critical behaviour for percolation in high dimensions}},
 FJournal = {{Communications in Mathematical Physics}},
 Journal = {{Commun. Math. Phys.}},
 ISSN = {0010-3616; 1432-0916/e},
 Volume = {128},
 Number = {2},
 Pages = {333--391},
 Year = {1990},
 Publisher = {Springer, Berlin/Heidelberg},
 MSC2010 = {60K35 82B43},
 Zbl = {0698.60100}
}

@Book{HeyHof17,
 Author = {M. {Heydenreich} and R. {van der Hofstad}},
 Title = {{Progress in high-dimensional percolation and random graphs}},
 FJournal = {{CRM Short Courses}},
 Journal = {{CRM Short Courses}},
 ISSN = {2522-5200},
 ISBN = {978-3-319-62472-3/hbk; 978-3-319-62473-0/ebook},
 Pages = {xii + 285},
 Year = {2017},
 Publisher = {Cham: Springer},
 MSC2010 = {60-02 60K35 82B43 05C80}
}

@article{HeyHofLasMat19,
       author = {{Heydenreich}, M. and {van der Hofstad}, R. and
         {Last}, G. and {Matzke}, K.},
        title = "{Lace Expansion and Mean-Field Behavior for the Random Connection Model}",
      journal = {arXiv e-prints},
     keywords = {Mathematics - Probability, 60K35, 82B43, 60G55},
         year = "2019",
        month = "Aug",
          eid = {arXiv:1908.11356},
        pages = {arXiv:1908.11356},
archivePrefix = {arXiv},
       eprint = {1908.11356},
 primaryClass = {math.PR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190811356H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}      
      
@article {jansen2016percolation,
    AUTHOR = {Jansen, S.},
     TITLE = {Continuum percolation for {G}ibbsian point processes with
              attractive interactions},
   JOURNAL = {Electron. J. Probab.},
  FJOURNAL = {Electronic Journal of Probability},
    VOLUME = {21},
      YEAR = {2016},
     PAGES = {Paper No. 47, 22 pp.}
}      
      
@article {kingman1967,
    AUTHOR = {Kingman, J. F. C.},
     TITLE = {Completely random measures},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {21},
      YEAR = {1967},
     PAGES = {59--78}
}

@article{LasZie17,
title={{On the Ornstein–Zernike equation for stationary cluster processes and the random connection model}}, 
volume={49}, 
DOI={10.1017/apr.2017.41}, 
number={4},
 journal={Adv. Appl. Probab.}, 
publisher={Cambridge University Press}, 
author={Last, G. and Ziesche, S.}, 
year={2017}, pages={1260–1287}
}

      
@book {malyshev-minlos,
    AUTHOR = {Malyshev, V. A. and Minlos, R. A.},
     TITLE = {Gibbs random fields. Cluster expansions},
    SERIES = {Mathematics and its Applications (Soviet Series)},
    VOLUME = {44},
      NOTE = { Translated from the Russian by R. Koteck\'{y} and P. Holick\'{y}},
 PUBLISHER = {Kluwer Academic Publishers Group, Dordrecht},
      YEAR = {1991},
     PAGES = {xiv+248}
}

@Book{MeeRoy96,
 Author = {R. {Meester} and R. {Roy}},
 Title = {{Continuum percolation}},
 FJournal = {{Cambridge Tracts in Mathematics}},
 Journal = {{Camb. Tracts Math.}},
 ISSN = {0950-6284},
 Volume = {119},
 ISBN = {0-521-47504-X},
 Pages = {x + 238},
 Year = {1996},
 Publisher = {Cambridge: Cambridge Univ. Press},
 MSC2010 = {60K35 60-02 60D05},
 Zbl = {0858.60092}
}

@article{OrnZer14,
  title={Accidental deviations of density and opalescence at the critical point of a single substance},
  author={{Ornstein}, L. S. and {Zernike}, F.},
  journal={Proc. Akad. Sci. (Amsterdam)},
  fjournal = {Koninklijke Nederlandse Akademie van Wetenschappen Proceedings Series B Physical Sciences},
  volume={17},
  pages = {793-806},
  year={1914},}
}

@Article{Pen93,
 Author = {M. D. {Penrose}},
 Title = {{On the spread-out limit for bond and continuum percolation}},
 FJournal = {{The Annals of Applied Probability}},
 Journal = {{Ann. Appl. Probab.}},
 ISSN = {1050-5164; 2168-8737/e},
 Volume = {3},
 Number = {1},
 Pages = {253--276},
 Year = {1993},
 Publisher = {Institute of Mathematical Statistics (IMS), Beachwood, OH/Bethesda, MD},
 MSC2010 = {60K35 60J80 82B43},
 Zbl = {0771.60097}
}

@Book{Sla06,
 Author = {G. {Slade}},
 Title = {{The lace expansion and its application. \'Ecole d'\'Et\'e de Probabilit\'es de Saint-Flour XXXIV -- 2004}},
 FJournal = {{Lecture Notes in Mathematics}},
 Journal = {{Lect. Notes Math.}},
 ISSN = {0075-8434; 1617-9692/e},
 Volume = {1879},
 ISBN = {3-540-31189-0/pbk},
 Pages = {xiii + 228},
 Year = {2006},
 Publisher = {Berlin: Springer},
 MSC2010 = {60-02 60K35 60G15 82B41},
 Zbl = {1113.60005}
}

@inproceedings{Ste76,
      author         = "Stell, G.",
      title          = "{Correlation Functions and their Generating Functionals:
                        General Relations with Applications to the Theory of
                        Fluids}",
      booktitle      = "{12th School of Modern Physics on Phase Transitions and
                        Critical Phenomena Ladek Zdroj, Poland, June 21-24, 2001}",
      year           = "1976",
      pages          = "205-258",
      SLACcitation   = "%%CITATION = INSPIRE-116315;%%"
}

@article{Ste96,
title = "Continuum theory of percolation and association",
journal = "Physica A",
fjournal = "Physica A: Statistical Mechanics and its Applications",
volume = "231",
number = "1",
pages = "1 - 19",
year = "1996",
issn = "0378-4371",
doi = "https://doi.org/10.1016/0378-4371(96)00079-9",
url = "http://www.sciencedirect.com/science/article/pii/0378437196000799",
author = "G. Stell",
}

@book {torquato-book,
    AUTHOR = {Torquato, S.},
     TITLE = {Random heterogeneous materials. Microstructure and macroscopic properties},
    SERIES = {Interdisciplinary Applied Mathematics},
    VOLUME = {16},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {2002},
     PAGES = {xxii+701}
}

 
----------------------------------------------------------------------------





@article {abraham-kunz77,
    AUTHOR = {Abraham, D. B. and Kunz, H.},
     TITLE = {Ornstein-{Z}ernike theory of classical fluids at low density},
   JOURNAL = {Phys. Rev. Lett.},
  FJOURNAL = {Physical Review Letters},
    VOLUME = {39},
      YEAR = {1977},
    NUMBER = {16},
     PAGES = {1011--1014}
}

@article {given-stell1990,
    AUTHOR = {Given, J. A. and Stell, G.},
     TITLE = {The {K}irkwood-{S}alsburg equations for random continuum
              percolation},
   JOURNAL = {J. Statist. Phys.},
  FJOURNAL = {Journal of Statistical Physics},
    VOLUME = {59},
      YEAR = {1990},
    NUMBER = {3-4},
     PAGES = {981--1018}
}

@article {kuna-tsagkaro2018,
    AUTHOR = {Kuna, T. and Tsagkarogiannis, D.},
     TITLE = {Convergence of density expansions of correlation functions and
              the {O}rnstein-{Z}ernike equation},
   JOURNAL = {Ann. Henri Poincar\'{e}},
  FJOURNAL = {Annales Henri Poincar\'{e}. A Journal of Theoretical and
              Mathematical Physics},
    VOLUME = {19},
      YEAR = {2018},
    NUMBER = {4},
     PAGES = {1115--1150}
}

@misc{ott-velenik2019,
  title={Asymptotics of correlations in the {I}sing model: a brief survey},
  author={Ott, S. and Velenik, Y.},
  howpublished = {Online preprint arXiv:1905.06207 [math.PR]},
  year={2019}
}


@Article{MeePenSar97,
 Author = {Meester, R. and Penrose, M. D. and Sarkar, A.},
 Title = {{The random connection model in high dimensions}},
 FJournal = {{Statistics \& Probability Letters}},
 Journal = {{Stat. Probab. Lett.}},
 ISSN = {0167-7152},
 Volume = {35},
 Number = {2},
 Pages = {145--153},
 Year = {1997},
 Publisher = {Elsevier (North-Holland), Amsterdam},

 MSC2010 = {60K35 82B43 60J80},
 Zbl = {0897.60096}
}

@Article{FitHof16,
 Author = {R. {Fitzner} and R. {van der Hofstad}},
 Title = {{Generalized approach to the non-backtracking lace expansion}},
 FJournal = {{Probability Theory and Related Fields}},
 Journal = {{Probab. Theory Relat. Fields}},
 ISSN = {0178-8051; 1432-2064/e},
 Volume = {169},
 Number = {3-4},
 Pages = {1041--1119},
 Year = {2017},
 Publisher = {Springer, Berlin/Heidelberg},
 MSC2010 = {82B41 82B43 60K35},
 Zbl = {1379.82010}
}

@Article{GupRao99,
 Author = {J. {Gupta} and B. {Rao}},
 Title = {{Van den Berg-Kesten inequality for the Poisson Boolean model for continuum percolation}},
 FJournal = {{Sankhy\=a. Series A. Methods and Techniques}},
 Journal = {{Sankhy\=a, Ser. A}},
 ISSN = {0581-572X},
 Volume = {61},
 Number = {3},
 Pages = {337--346},
 Year = {1999},
 Publisher = {Indian Statistical Institute, Calcutta},
 MSC2010 = {60K35 82B43},
 Zbl = {0977.60100}
}

@Article{HeyHofSak08,
 Author = {M. {Heydenreich} and R. {van der Hofstad} and A. {Sakai}},
 Title = {{Mean-field behavior for long- and finite range Ising model, percolation and self-avoiding walk}},
 FJournal = {{Journal of Statistical Physics}},
 Journal = {{J. Stat. Phys.}},
 ISSN = {0022-4715; 1572-9613/e},
 Volume = {132},
 Number = {6},
 Pages = {1001--1049},
 Year = {2008},
 Publisher = {Springer US, New York, NY},
 MSC2010 = {82B41 82B43 60K35 82B27},
 Zbl = {1152.82007}
}


@article{vdB96,
 Author = {Berg, J. van den},
 Title = {{A note on disjoint-occurrence inequalities for marked Poisson point processes}},
 FJournal = {{Journal of Applied Probability}},
 Journal = {{J. Appl. Probab.}},
 ISSN = {0021-9002; 1475-6072/e},
 Volume = {33},
 Number = {2},
 Pages = {420--426},
 Year = {1996},
 Publisher = {Applied Probability Trust, Sheffield},
 MSC2010 = {60E15 60G55 82B43 60K35},
 Zbl = {0860.60013}
}


@Book{LasPen17,
 Author = {G. {Last} and M. D. {Penrose}},
 Title = {{Lectures on the Poisson process}},
 FJournal = {{Institute of Mathematical Statistics Textbooks}},
 Journal = {{IMS Textb.}},
 Volume = {7},
 ISBN = {978-1-107-45843-7/pbk; 978-1-107-08801-6/hbk; 978-1-316-10447-7/ebook},
 Pages = {xx + 293},
 Year = {2018},
 Publisher = {Cambridge: Cambridge University Press},
 MSC2010 = {60-02 60G55 60G10 60D05},
 Zbl = {1392.60004}
}


@book {Gri99,
    AUTHOR = {Grimmett, G.},
     TITLE = {Percolation},
    SERIES = {Grundlehren der Mathematischen Wissenschaften [Fundamental
              Principles of Mathematical Sciences]},
    VOLUME = {321},
   EDITION = {2nd},
 PUBLISHER = {Springer-Verlag, Berlin},
      YEAR = {1999},
     PAGES = {xiv+444},
      ISBN = {3-540-64902-6},
       DOI = {10.1007/978-3-662-03981-6},
       URL = {https://doi.org/10.1007/978-3-662-03981-6},
}



@Book{BolRio06,
 Author = {B. {Bollob\'as} and O. {Riordan}},
 Title = {{Percolation}},
 ISBN = {0-521-87232-4/hbk},
 Pages = {x + 323},
 Year = {2006},
 Publisher = {Cambridge: Cambridge University Press},
 MSC2010 = {60-01 82-01 60K35 82B43},
 Zbl = {1118.60001}
}

@InCollection{Tan96,
 Author = {H. {Tanemura}},
 Title = {{Critical behavior for a continuum percolation model}},
 BookTitle = {{Probability theory and mathematical statistics. Proceedings of the seventh Japan-Russia symposium, Tokyo, Japan, July 26--30, 1995}},
 ISBN = {981-02-2426-5/hbk},
 Pages = {485--495},
 Year = {1996},
 Publisher = {Singapore: World Scientific},
 MSC2010 = {60K35 82B43},
 Zbl = {0961.60095}
}

@article{AizBar91,
 Author = {D. {Barsky} and M. {Aizenman}},
 Title = {{Percolation critical exponents under the triangle condition}},
 FJournal = {{The Annals of Probability}},
 Journal = {{Ann. Probab.}},
 ISSN = {0091-1798; 2168-894X/e},
 Volume = {19},
 Number = {4},
 Pages = {1520--1536},
 Year = {1991},
 Publisher = {Institute of Mathematical Statistics (IMS), Beachwood, OH/Bethesda, MD},
 MSC2010 = {60K35 82B43 34A40 60D05 82B27},
 Zbl = {0747.60093}
}

@article{AizNew84,
 Author = {M. {Aizenman} and C. {Newman}},
 Title = {{Tree graph inequalities and critical behavior in percolation models}},
 FJournal = {{Journal of Statistical Physics}},
 Journal = {{J. Stat. Phys.}},
 ISSN = {0022-4715; 1572-9613/e},
 Volume = {36},
 Pages = {107--144},
 Year = {1984},
 Publisher = {Springer US, New York, NY},
 MSC2010 = {60K35 82B43},
 Zbl = {0586.60096}
}


@Article{FitHof17,
 Author = {R. {Fitzner} and R. {van der Hofstad}},
 Title = {{Mean-field behavior for nearest-neighbor percolation in \(d>10\)}},
 FJournal = {{Electronic Journal of Probability}},
 Journal = {{Electron. J. Probab.}},
 ISSN = {1083-6489/e},
 Volume = {22},
 Pages = {65},
 Note = {Id/No 43},
 Year = {2017},
 Publisher = {University of Washington, Department of Mathematics, Seattle, WA; Duke University, Department of Mathematics, Durham, NC},
 MSC2010 = {60K35 82B43 82B27},
 Zbl = {1364.60130}
}



@article{LasPenZuy17,
 Author = {G. {Last} and M. D. {Penrose} and S. {Zuyev}},
 Title = {{On the capacity functional of the infinite cluster of a Boolean model}},
 FJournal = {{The Annals of Applied Probability}},
 Journal = {{Ann. Appl. Probab.}},
 ISSN = {1050-5164; 2168-8737/e},
 Volume = {27},
 Number = {3},
 Pages = {1678--1701},
 Year = {2017},
 Publisher = {Institute of Mathematical Statistics (IMS), Beachwood, OH/Bethesda, MD},
 MSC2010 = {60K35 60D05},
 Zbl = {1373.60160}
}

@article{Pen91,
 Author = {M. D. {Penrose}},
 Title = {{On a continuum percolation model}},
 FJournal = {{Advances in Applied Probability}},
 Journal = {{Adv. Appl. Probab.}},
 ISSN = {0001-8678},
 Volume = {23},
 Number = {3},
 Pages = {536--556},
 Year = {1991},
 Publisher = {Applied Probability Trust, Sheffield; Cambridge University Press, Cambridge},
 MSC2010 = {60K35 82B43},
 Zbl = {0729.60106}
}

@article{Mee95,
 Author = {R. {Meester}},
 Title = {{Equality of critical densities in continuum percolation}},
 FJournal = {{Journal of Applied Probability}},
 Journal = {{J. Appl. Probab.}},
 ISSN = {0021-9002; 1475-6072/e},
 Volume = {32},
 Number = {1},
 Pages = {90--104},
 Year = {1995},
 Publisher = {Applied Probability Trust, Sheffield},
 MSC2010 = {60K35 82B43 60G55},
 Zbl = {0816.60098}
}

@article{BroHam57,
 Author = {S. {Broadbent} and J. {Hammersley}},
 Title = {{Percolation processes. I: Crystals and mazes}},
 FJournal = {{Proceedings of the Cambridge Philosophical Society}},
 Journal = {{Proc. Camb. Philos. Soc.}},
 ISSN = {0008-1981},
 Volume = {53},
 Pages = {629--641},
 Year = {1957},
 Publisher = {Cambridge Philosophical Society},
 Zbl = {0091.13901}
}

@Article{Gil61,
 Author = {E. {Gilbert}},
 Title = {{Random plane networks}},
 FJournal = {{Journal of the Society for Industrial \& Applied Mathematics}},
 Journal = {{J. Soc. Ind. Appl. Math.}},
 ISSN = {0368-4245},
 Volume = {9},
 Pages = {533--543},
 Year = {1961},
 Publisher = {Society for Industrial \& Applied Mathematics, Philadelphia},
 Zbl = {0112.09403}
}

@Article{Har90,
 Author = {T. {Hara}},
 Title = {{Mean-field critical behaviour for correlation length for percolation in high dimensions}},
 FJournal = {{Probability Theory and Related Fields}},
 Journal = {{Probab. Theory Relat. Fields}},
 ISSN = {0178-8051; 1432-2064/e},
 Volume = {86},
 Number = {3},
 Pages = {337--385},
 Year = {1990},
 Publisher = {Springer, Berlin/Heidelberg},
 MSC2010 = {60K35 82B43},
 Zbl = {0685.60102}
}

@article{HarHofSla03,
 Author = {T. {Hara} and R. {van der Hofstad} and G. {Slade}},
 Title = {{Critical two-point functions and the lace expansion for spread-out high-dimensional percolation and related models}},
 FJournal = {{The Annals of Probability}},
 Journal = {{Ann. Probab.}},
 ISSN = {0091-1798; 2168-894X/e},
 Volume = {31},
 Number = {1},
 Pages = {349--408},
 Year = {2003},
 Publisher = {Institute of Mathematical Statistics (IMS), Beachwood, OH/Bethesda, MD},
 MSC2010 = {82B41 82B27 82B43 60K35},
 Zbl = {1044.82006}
}

@article{Har08,
 Author = {T. {Hara}},
 Title = {{Decay of correlations in nearest-neighbor self-avoiding walk, percolation, lattice trees and animals}},
 FJournal = {{The Annals of Probability}},
 Journal = {{Ann. Probab.}},
 ISSN = {0091-1798; 2168-894X/e},
 Volume = {36},
 Number = {2},
 Pages = {530--593},
 Year = {2008},
 Publisher = {Institute of Mathematical Statistics (IMS), Beachwood, OH/Bethesda, MD},
 MSC2010 = {82B27 82B41 82B43},
 Zbl = {1142.82006}
}


@article{KozNac11,
 Author = {G. {Kozma} and A. {Nachmias}},
 Title = {{Arm exponents in high dimensional percolation}},
 FJournal = {{Journal of the American Mathematical Society}},
 Journal = {{J. Am. Math. Soc.}},
 ISSN = {0894-0347; 1088-6834/e},
 Volume = {24},
 Number = {2},
 Pages = {375--409},
 Year = {2011},
 Publisher = {American Mathematical Society (AMS), Providence, RI},
 MSC2010 = {60K35 82B43},
 Zbl = {1219.60085}
}

@Article{KozNac09,
 Author = {G. {Kozma} and A. {Nachmias}},
 Title = {{The Alexander-Orbach conjecture holds in high dimensions}},
 FJournal = {{Inventiones Mathematicae}},
 Journal = {{Invent. Math.}},
 ISSN = {0020-9910; 1432-1297/e},
 Volume = {178},
 Number = {3},
 Pages = {635--654},
 Year = {2009},
 Publisher = {Springer, Berlin/Heidelberg},
 MSC2010 = {82B43 82B41 82B27},
 Zbl = {1180.82094}
}



@article{BorChaHofSlaSpe05,
 Author = {C. {Borgs} and J. {Chayes} and R. {van der Hofstad} and G. {Slade} and J. {Spencer}},
 Title = {{Random subgraphs of finite graphs. II: The lace expansion and the triangle condition}},
 FJournal = {{The Annals of Probability}},
 Journal = {{Ann. Probab.}},
 ISSN = {0091-1798; 2168-894X/e},
 Volume = {33},
 Number = {5},
 Pages = {1886--1944},
 Year = {2005},
 Publisher = {Institute of Mathematical Statistics (IMS), Beachwood, OH/Bethesda, MD},
 MSC2010 = {05C80 60K35 82B43},
 Zbl = {1079.05087}
}

@Article{BefDum13,
 Author = {V. {Beffara} and H. {Duminil-Copin}},
 Title = {{Planar percolation with a glimpse of Schramm-Loewner evolution}},
 FJournal = {{Probability Surveys}},
 Journal = {{Probab. Surv.}},
 ISSN = {1549-5787/e},
 Volume = {10},
 Pages = {1--50},
 Year = {2013},
 Publisher = {Sponsored by Institute of Mathematical Statistics, Beachwood, OH; Bernoulli Society},
 MSC2010 = {60K35 60J67},
 Zbl = {1283.60118}
}

@Book{Wer09,
 Author = {W. {Werner}},
 Title = {{Percolation et mod\`ele d'Ising}},
 FJournal = {{Cours Sp\'ecialis\'es (Paris)}},
 Journal = {{Cours Sp\'ec. (Paris)}},
 ISSN = {1284-6090},
 Volume = {16},
 ISBN = {978-2-85629-276-1/hbk},
 Pages = {vi + 161},
 Year = {2009},
 Publisher = {Paris: Soci\'et\'e Math\'ematique de France},
 Language = {French},
 MSC2010 = {82-02 82B43 82B44},
 Zbl = {1206.82002}
}

@Book{Pen03,
 Author = {M. D. {Penrose}},
 Title = {{Random geometric graphs}},
 FJournal = {{Oxford Studies in Probability}},
 Journal = {{Oxf. Stud. Probab.}},
 Volume = {5},
 ISBN = {0-19-850626-0/hbk},
 Pages = {xiii + 330},
 Year = {2003},
 Publisher = {Oxford: Oxford University Press},
 MSC2010 = {60D05 05C80 60C05 60K35 60-02},
 Zbl = {1029.60007}
}

@article{Pen16,
 Author = {M. D. {Penrose}},
 Title = {{Connectivity of soft random geometric graphs}},
 FJournal = {{The Annals of Applied Probability}},
 Journal = {{Ann. Appl. Probab.}},
 ISSN = {1050-5164; 2168-8737/e},
 Volume = {26},
 Number = {2},
 Pages = {986--1028},
 Year = {2016},
 Publisher = {Institute of Mathematical Statistics (IMS), Beachwood, OH/Bethesda, MD},
 MSC2010 = {05C80 60D05 05C40 60K35},
 Zbl = {1339.05369}
}


@mastersthesis{vdBru03,
author ={Brug, T. van de},
title={{The random connection model: Construction, central limit theorem and asymptotic connectivity}},
school={Vrije Universiteit Amsterdam},
year={2003}
}


@Book{Tor02,
 Author = {S. {Torquato}},
 Title = {{Random heterogeneous materials. Microstructure and macroscopic properties}},
 FJournal = {{Interdisciplinary Applied Mathematics}},
 Journal = {{Interdiscip. Appl. Math.}},
 ISSN = {0939-6047},
 Volume = {16},
 ISBN = {0-387-95167-9},
 Pages = {xxi + 701},
 Year = {2002},
 Publisher = {New York, NY: Springer},
 MSC2010 = {74-02 74A40 74E05 74A60 74E30 74Q15},
 Zbl = {0988.74001}
}


@article{Tor12,
author = {Torquato, S. },
title = {Effect of dimensionality on the continuum percolation of overlapping hyperspheres and hypercubes},
journal = {J. Chem. Phys.},
volume = {136},
number = {5},
pages = {054106},
year = {2012},
doi = {10.1063/1.3679861},
URL = {         https://doi.org/10.1063/1.3679861},
eprint = {       https://doi.org/10.1063/1.3679861   }
}

@Book{DhaJoa88,
 Author = {S. {Dharmadhikari} and K. {Joag-dev}},
 Title = {{Unimodality, convexity and applications}},
 ISBN = {0-12-214690-5},
 Pages = {xiii + 278},
 Year = {1988},
 Publisher = {London: Academic Press, Inc.},
 MSC2010 = {62E10 60E05 60-02 62-02 26A51 62H05},
 Zbl = {0646.62008}
}

@article{ChiSte89,
author = {Chiew,Y. C.  and Stell,G. },
title = {Connectivity and percolation of randomly centered spheres: Correction to the Percus–Yevick approximation},
journal = {The Journal of Chemical Physics},
volume = {90},
number = {9},
pages = {4956-4959},
year = {1989}
}

@book{hansen2013theory,
  title={Theory of Simple Liquids: with Applications to Soft Matter},
  author={Hansen, J. P. and McDonald, I. R.},
  publisher={Academic Press},
  year={2013}
}

@article{OgaTan89,
author = {Ogata,Y.  and Tanemura,M. },
title = {LIKELIHOOD ESTIMATION  OF  SOFT-CORE 
INTERACTION POTENTIALS FOR 
{G}IBBSIAN  POINT  PATTERNS},
journal = {Ann.  Inst.  Statist.  Math. },
volume = {41},
number = {3},
pages = {583-600},
year = {1989}
}
@inproceedings{Betsch2021OnTU,
  title={On the uniqueness of {G}ibbs distributions with a non-negative and subcritical pair potential},
  author={S. Betsch and G. Last},
  year={2021}
}
